Associated production of a Z boson and a b-jet in ATLAS

The current uncertainty on the parametrization of the partonic content of the proton (PDF's) affects the potential for the discovery of new physics at LHC. The study of Z boson production in association with a b-jet can considerably reduce such uncertainty. In addition, this process represents a background both to the search for the Higgs boson and for SUSY particles. We present an update, based on the full simulation data sample produced for the Rome Physics Workshop, of a preliminary study in the case where the Z boson decays in mu+ mu-.

==> bibliografia.tex <==
\begin{thebibliography}
\bibitem{athena}  nome, \emph{titolo} 
\bibitem{c++}  nome, \emph{titolo} 
\bibitem{ipatrec}  nome, \emph{titolo} 
\bibitem{muid}  nome, \emph{titolo} 
\bibitem{spect}  nome, \emph{titolo} 
\bibitem{muonbox}  nome, \emph{titolo} 
\bibitem{ptdr}  nome, \emph{titolo} 
%\bibitem{nome}  nome, \emph{titolo} 
\end{thebibliography}



==> doccut.tex <==
\section{Moore}
Moore (Muon Object Oriented Reconstruction) is a track reconstruction 
package for the Muon Spectrometer. 
A detailed description of Moore is available elsewhere~\cite{Moore}.
 
Moore takes as input collections of digits or clusters inside the 
Muon Spectrometer (CSC, MDT, RPC, TGC)  and outputs 
fitted reconstructed tracks whose parameters are referred 
at the first measured point of the Muon Spectrometer.
 
The reconstruction is performed in several steps and each step is 
driven by an ATHENA top-Algorithm module (MooMakeXXX).
% see Figure~\ref{fig:Mooscheme}.  
%\begin{figure}[tp]
%\begin{center}
%\epsfig{file=moorescheme.eps,width=\textwidth}
%\caption[]{Data access from the Moore Algorithms.}
%\label{fig:Mooscheme}
%\end{center}
%\end{figure}
Each algorithm is independent, i.e. it retrieves objects created 
by the previous modules from StoreGate and it builds a
transient object to be recorded in StoreGate where it is available 
for the subsequent algorithms. 
The only link between algorithms are the transient objects, in such a way that the 
algorithms depend on transient objects but transient objects do not
depend on algorithms. 
The decoupling between data and algorithms and the natural step 
sequence of algorithm performing the reconstruction gives
the opportunity to plug-in different reconstruction algorithms at 
run time.

As it is now the overall reconstruction starts from the searches for $\phi$ 
regions of activity and builds PhiSegments (MooMakePhiSegments). For each  
$\phi$-Segment, the associated MDTs are found and a {\it crude}
 RZSegment is built (this is essentially a collection of z hits) 
(MooMakeRZSegments).

Inside the MDTs the drift distance is calculated from the drift time, 
by applying various corrections: such as the TOF, the second coordinate, 
the propagation along the wire, the Lorenz effect.
From the 4 tangential lines the best one is found.
All the MDT segments of the outer station are combined with 
those of the Middle layer.
The MDT hits of each combination are added to the phi-hits of the $\phi$ 
Segment, forming outer track candidates. 
All the successfully fitted candidates are kept for further processing 
(MooMakeRoads).

The successfull outer track is subsequentely used to associate 
inner station MDT hits. A final track is defined as a successfully 
fitted collection of trigger hits and MDT hits from at least 
two layers (MooMakeTracks). 
The parameters of the fitted track are referred to the first measured 
point of the Muon Spectrometer.

When dealing with data already selected by the trigger the first two steps
(MooMakePhiSegments) and (MooMakeRZSegments) can be substitute with {\it ad  
hoc} makers that seed the track search in the regions selected by the trigger.
  



==> headings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%                                                                     %
% Macintosh:     Macintosh HD:Paolo:/u1/pvalente/tesi2e/headings.tex  %
%                                                                     %
% HP-UX hpserver:                   /u1/pvalente/tesi2e/headings.tex  %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                 Tesi di Laurea di Paolo Valente                     %  
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
%\renewcommand{\chaptermark}[1]{\markboth{{\bf\large\@chapapp\ \thechapter .\ } #1}}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}} 
\renewcommand{\sectionmark}[1]{\markright{\bf\large\thesection\ #1}}
\makeatother

\lhead[\fancyplain{}{\bf\large\thepage}]{\fancyplain{}{\it\large\rightmark}}
\rhead[\fancyplain{}{\it\large\leftmark}]{\fancyplain{}{\bf\large\thepage}}
\lfoot{\fancyplain{\bf\large\thepage}{}}



==> headings1.tex <==
\makeatletter
\renewcommand{\chaptermark}[1]{\markboth{{} #1}}
%                                     {{} #1}} 
\renewcommand{\sectionmark}[1]{\markright{{\bf\large\thesection\ } #1}}
%\makeatother

\lhead[\fancyplain{}{\bf\large\thepage}]{\fancyplain{}{\it\large\rightmark}}
\rhead[\fancyplain{}{\it\large\leftmark}]{\fancyplain{}{\bf\large\thepage}}
\cfoot{\fancyplain{\bf\large\thepage}{}}


==> hyphenations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%                                                                     %
% HP-UX hpserver:/nfs/kloe02/kloe08/data/users/sciascia/tesi/tesi.tex %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                 Tesi di Laurea di Barbara Sciascia                  %  
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hyphenation{par-ti-cel-la par-ti-cel-le ele-men-ta-re ele-men-ta-ri}
\hyphenation{vio-la-zio-ne co-me con-se-guen-za quin-di han-no stra-nez-za}
\hyphenation{dop-piet-to dop-piet-ti de-ca-di-men-to de-ca-di-men-ti}
\hyphenation{con-ser-va-zio-ne si-mil-men-te co-niu-ga-zio-ne}
\hyphenation{se-mi-le-pto-ni-co se-mi-le-pto-ni-ci lep-to-ni-ci}
\hyphenation{ha-mil-to-nia-na au-to-sta-to au-to-sta-ti}
\hyphenation{so-vrap-po-si-zio-ne so-vrap-po-si-zio-ni}
\hyphenation{con-fi-gu-ra-zio-ne con-fi-gu-ra-zio-ni}
\hyphenation{tran-si-zio-ne tran-si-zio-ni piom-bo}
\hyphenation{spe-ri-men-ta-le spe-ri-men-ta-li spe-ri-men-tal-men-te}
\hyphenation{con-si-de-ra-re in-te-ra-zio-ne in-te-ra-zio-ni}
\hyphenation{cor-re-zio-ne cor-re-zio-ni mas-sa piom-bo}
\hyphenation{in-tro-dot-to in-tro-dot-ta in-tro-dot-ti in-tro-dot-te}
\hyphenation{pos-so-no es-se-re que-stio-ne}
\hyphenation{es-pri-me-re es-pres-sio-ne es-pres-sio-ni}
\hyphenation{es-pres-so es-pres-si es-pres-sa es-pres-se}
\hyphenation{in-tro-du-zio-ne in-ter-pre-ta-to in-ter-pre-ta-ti}
\hyphenation{for-ma-li-smo for-ma-li-smi her-mi-tia-no her-mi-tia-ni}
\hyphenation{coor-di-na-ta coor-di-na-te coef-fi-cien-te coef-fi-cien-ti}
\hyphenation{de-ter-mi-na-re ot-te-ne-re im-ma-gi-na-rio}
\hyphenation{im-ma-gi-na-rio im-ma-gi-na-ri im-ma-gi-na-ria im-ma-gi-na-rie} 
\hyphenation{la-scian-do evi-den-te-men-te na-tu-ral-men-te}
\hyphenation{Ha-mil-to-nia-na sta-ti ca-na-li co-mu-ni in-ter-fe-ren-za}
\hyphenation{cam-pio-na-tu-ra pro-ble-ma u-san-do mol-te-pli-ci-ta}
\hyphenation{io-niz-za-zio-ne io-niz-za-re u-sa-to}
\hyphenation{in-di-vi-du-are ci-ne-ma-ti-ci}
\hyphenation{con-si-de-ran-do con-te-nu-ti vo-lu-me fi-du-cia-le}
\hyphenation{dis-cre-te de-fi-ni-to ef-fi-cien-za co-stru-zio-ne}
\hyphenation{ca-me-ra de-ri-va e-spe-ri-men-to que-sto ca-pi-to-lo}
\hyphenation{mac-chi-na u-ni-co in-for-ma-zio-ni pro-ve-nien-ti}
\hyphenation{ac-cu-ra-tez-za fo-to-me-tro ca-li-bra-zio-ne re-la-zio-ni}
\hyphenation{de-ter-mi-na-zio-ne in-va-rian-za mi-su-ra pro-du-zio-ne}
\hyphenation{tar-ghet-ta de-di-ca-to mo-du-lo con-tie-ne som-ma-ti}
\hyphenation{piat-ti ge-o-me-tri-ca ri-ge-ne-ra-to spe-ri-men-ta-zio-ne}


==> lista.tex <==
K.Mair 
Technische Universität Wien (TU) 

                 European Organization for Nuclear Research (CERN)
		 A.Nairz
		 
		 A.Poppleton
		 
                 European Organization for Nuclear Research (CERN)
		 
		 S.Rosati
		 
                 European Organization for Nuclear Research (CERN)
		 
		 D.Adams
		 Brookhaven National Laboratory (BNL)
		 K.Assamagan
		 
		 
		 Goldfarb
		 University of Michigan
		 
		 Università degli Studi di Lecce 
		 
		 Lawrence Berkeley National Laboratory (LBNL) 
		 Università di Napoli "Federico II" 
		 Terza Università di Roma
		
                 Aristotle University of Thessaloníki 


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%                                                                     %
% Macintosh:     Macintosh HD:Paolo:/u1/pvalente/tesi2e/macros2e.tex  %
%                /scrtch1/kloe/barbara/tesi/BLaurea                   %
% HP-UX hpserver:                   /u1/pvalente/tesi2e/macros2e.tex  %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                 Tesi di Laurea di Barbara Sciascia                  %  
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\fnum@figure{{\bf Figura \thefigure}\footnotesize}
\def\fnum@table{{\bf Tabella \thetable}\footnotesize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@chapapp{Capitolo}

\def\@makechapterhead#1{\vspace*{50\p@}
%        \vspace*{50\p@}
  {\parindent \z@ \centering \reset@font
    \ifnum \c@secnumdepth >\m@ne
      \LARGE\bfseries \@chapapp{} \thechapter 
      \par
     \vskip 20\p@
   \fi
   \Huge \bfseries #1\par
    \nobreak
    \vskip 40\p@
  }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\chaptermark}[1]{\markboth{\thechapter. #1}{}}
%\newcommand{\sectionmark}[1]{\markright{\thesection. #1}}









%\def\@schapter#1{\if@twocolumn
%                  \@topnewpage[\@makeschapterhead{#1}]%
%                 \else
%                   \@makeschapterhead{#1}%
%                   \@afterheading
%                 \fi}
%\def\@makeschapterhead#1{%
%  \vspace*{50\p@}%
%  {\parindent \z@ \centering
%    \reset@font
%    \Huge \bfseries  #1\par
%    \nobreak
%    \vskip 40\p@
% }}
%
\def\tableofcontents{\@restonecolfalse\if@twocolumn\@restonecoltrue\onecolumn
  \fi\chapter*{Indice\@mkboth {\bf {Indice}} {\bf{Indice}}}
  \@starttoc{toc}\if@restonecol\twocolumn\fi}
%
\def\thebibliography#1{\chapter*{Bibliografia\addcontentsline{toc}{chapter}
  {Bibliografia}\@mkboth
  {\bf Bibliografia}{\bf Bibliografia}}\list
  {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
    \advance\leftmargin\labelsep
    \usecounter{enumi}}
    \def\newblock{\hskip .11em plus .33em minus -.07em}
    \sloppy
    \sfcode`\.=1000\relax}
%
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\scr                 {\scriptstyle}
\def\sscr                {\scriptscriptstyle}
\def\rmscr               {\rm \scriptstyle}
\def\rmsscr              {\rm \scriptscriptstyle}

%

\newcommand{\e}[1]       {\mbox{$\cdot 10^{\sscr #1} $}}
\newcommand{\Darrow}     {\mbox{\rlap{$\leftarrow$}\raisebox{0.6ex}{$\rightarrow$}}}
\newcommand{\bra}[1]     {\mbox{$\langle #1|$}}
\newcommand{\ket}[1]     {\mbox{$| #1\rangle$}}
\newcommand{\Bra}[1]     {\mbox{$\left\langle #1\right|$}}
\newcommand{\Ket}[1]     {\mbox{$\left| #1\right\rangle$}}
\newcommand{\braket}[3]  {\mbox{$\langle #1|#2|#3\rangle$}}
\newcommand{\Braket}[3]  {\mbox{$\left\langle #1\left|#2\right|#3\right\rangle$}}
\newcommand{\scalare}[2]  {\mbox{$\langle #1|#2\rangle$}}
\newcommand{\Scalare}[2]  {\mbox{$\left\langle #1\left|#2\right\rangle$}}
\newcommand{\slashed}[1] {\mbox{\rlap{\hbox{/}}#1}}
\newcommand{\GIm}[1]     {\Im{\frak{m}\left(#1\right)}}
\newcommand{\GRe}[1]     {\Re{\frak{e}\left(#1\right)}}
\newcommand{\duplet}[2]  {\left({\rlap{\raisebox{-1.5ex}{#2}}
                          \raisebox{1.5ex}{#1}}\right)}
\newcommand{\triplet}[3]  {\left({\rlap{\raisebox{-2.0ex}{#3}}
                          \raisebox{0ex}{#2}}{\raisebox{2.0ex}{#1}}\right)}			  
			  
%
\newcommand{\taumeno}    {\mbox{${\tau}^{\sscr -}$}}
\newcommand{\nutau}      {\mbox{${\nu}_{\sscr \tau}$}}
\newcommand{\zzero}      {\mbox{${\rm Z}^{\sscr 0}$}}
\newcommand{\zalf}      {\mbox{${\rm Z}^{\sscr {\alpha}}$}}
\newcommand{\epiu}      {\mbox{${\rm e}^{\sscr +}$}}
\newcommand{\emeno}     {\mbox{${\rm e}^{\sscr -}$}}
\newcommand{\mupiu}     {\mbox{${\mu}^{\sscr +}$}}
\newcommand{\mumeno}    {\mbox{${\mu}^{\sscr -}$}}
\newcommand{\mumenopiu} {\mbox{$\mu^{\sscr \mp}$}}
\newcommand{\emenopiu}  {\mbox{${\rm e}^{\sscr \mp}$}}
\newcommand{\pmenopiu}  {\mbox{${\pi}^{\sscr \mp}$}}
\newcommand{\mupiumeno} {\mbox{$\mu^{\sscr \pm}$}}
\newcommand{\epiumeno}  {\mbox{${\rm e}^{\sscr \pm}$}}
\newcommand{\ppiumeno}  {\mbox{${\pi}^{\sscr \pm}$}}
\newcommand{\nue}       {\mbox{${\nu}_{\rm\sscr e}$}}
\newcommand{\numu}      {\mbox{${\nu}_{\sscr \mu}$}}
\newcommand{\ppiu}   {\mbox{${\pi}^{\rmsscr +} $}}
\newcommand{\pmeno}  {\mbox{${\pi}^{\rmsscr -} $}}
\newcommand{\pzero}  {\mbox{${\pi}^{\rmsscr 0} $}}
\newcommand{\kpiu}   {\mbox{${\rm K}^{\rmsscr +} $}}
\newcommand{\kmeno}  {\mbox{${\rm K}^{\rmsscr -} $}}
\newcommand{\kzero}  {\mbox{${\rm K}^{\rmsscr 0} $}}
\newcommand{\kzerob} {\mbox{${\bar{\rm K}}^{\rmsscr 0} $}}
\newcommand{\bzero}  {\mbox{${\rm B}^{\rmsscr 0} $}}
\newcommand{\bzerob} {\mbox{${\bar{\rm B}}^{\rmsscr 0} $}}
\newcommand{\kl}     {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr L} $}}
\newcommand{\ks}     {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr S} $}}

\newcommand{\GammaS} {\Gamma_{\rm\sscr S}}
\newcommand{\GammaL} {\Gamma_{\rm\sscr L}}
\newcommand{\gammaS} {\gamma_{\rm\sscr S}}
\newcommand{\gammaL} {\gamma_{\rm\sscr L}}

\newcommand{\kuno}   {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr 1} $}}
\newcommand{\kdue}   {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr 2} $}}
\newcommand{\kzerokzerob} {\ensuremath{\kzero - \kzerob}}
\newcommand{\MS}          {\mbox{$\cal MS$}}
\newcommand{\La}          {\mbox{${\cal L}$}}
\newcommand{\CP}          {\ensuremath{\mbox{$\cal CP$}}}
\newcommand{\T}           {\mbox{$\cal T$}}
\newcommand{\CPT}         {\ensuremath{\mbox{$\cal CPT$}}}
\newcommand{\C}           {\mbox{$\cal C$}}
\newcommand{\Pa}          {\mbox{$\cal P$}}
\newcommand{\Hsuno}    {\mbox{${\cal H}_{\sscr |\Delta S|=1}$}} 
\newcommand{\Hsdue}    {\mbox{${\cal H}_{\sscr |\Delta S|=2}$}}
\newcommand{\imez}     {\mbox{$\frac{\scr i}{\rm\scr 2}$}}
\newcommand{\unotre}    {\mbox{$\sqrt{\frac{\rm\sscr 1}{\rm\sscr 3}}$}}
\newcommand{\duetre}    {\mbox{$\sqrt{\frac{\rm\sscr 2}{\rm\sscr 3}}$}}
\newcommand{\kls}       {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr L,S} $}}
\newcommand{\phifa}      {$\phi$-{\it factory\/}}   
\newcommand{\Da}         {DA$\Phi$NE}
\newcommand{\epiuemeno}  {\mbox{${\rm e}^{\sscr +} {\rm e}^{\sscr -}$}}

\newcommand{\lsim}   {\mbox{\rlap{\raisebox{-1ex}{$\sim$}}$<$}}
\newcommand{\gsim}   {\mbox{\rlap{\raisebox{-1ex}{$\sim$}}$>$}}

\newcommand{\Me}     {\mbox{${\rm CH}_{\sscr 4}$}}
\newcommand{\iso}    {\mbox{$i{\rm C}_{\sscr 4}{\rm H}_{\sscr 10}$}}
\newcommand{\CO}     {\mbox{${\rm CO}_{\sscr 2}$}}

\newcommand{\epseps} {\mbox{$\frac{\epsilon{\rm\sscr '}}{\epsilon}$}}
\newcommand{\eps}    {\mbox{$\epsilon{\rm\sscr '}$}}

% Paolo Valente





==> monica.tex <==
%\if@twoside
%\def\ps@headings{\let\@mkboth\markboth
%\def\@oddfoot{\tensf\thepage}\def\@evenfoot{}
%\def\@evenhead{\rule[-8pt]{\texwidth}{0.5pt}\hskip-\texwidth
%{\tensf \thepage}\hfil {\tensf\leftmark}}
%\def\@oddhead{\rule[-8pt]{\texwidth}{0.5pt}\hskip-\texwidth
%{\sl \rightmark}\hfil {\tensf\thepage}}
%\def\chaptermark##1{\markboth {{ifnum \c@secnumdepth >\m@ne
%   \@chaapp\ \it\thechapter. \ \fi##1}}{}}
%\def\sectionmark##1{\markright {{ifnum \c@secnumdepth >\z@
%    \@thesection. \ \ fi ##1}}}}

%\fancyhead{}
\fancyhf{}
\renewcommand{\chaptermark}[1]{\markboth{\thechapter. #1}{}}
\renewcommand{\sectionmark}[1]{\markright{\thesection. #1}{}}
\lhead[\bfseries\sl{\rightmark}]{\bf \sl{ ATLAS}}
\rhead[\bf \sl{Tesi di Laurea }]{\bfseries\sl\footnotesize{\leftmark}}
%\lfoot[\bfseries\thepage]{}
%\rfoot[]{\bfseries\thepage}
\cfoot[\thepage]{\thepage}  

    
    
    
\newcommand{\Jn}   {\mbox{${\rm J}^{\rmsscr N}_{\rmsscr{\alpha } $}}}
\newcommand{\Jcp}  {\mbox{${\rm J}^{\rmsscr {C+}}_{\rmsscr{\alpha }} $}}
\newcommand{\Jc}   {\mbox{${\rm J}^{\rmsscr C}_{\rmsscr{\alpha } $}}}
\newcommand{\Jem}  {\mbox{${\rm J}^{\rmsscr {em}}_{\rmsscr{\alpha } $}}}

\newcommand{\A}    {\mbox{${\rm A}^{\rmsscr{\alpha } } $}}
\newcommand{\co}  {\mbox{${\cos{\theta}_{w}} $}} 
\newcommand{\se}  {\mbox{${\sin{\theta}_{w}} $}}
\newcommand{\Wp}  {\mbox{${\rm W}^{\rmsscr {+{\alpha}}} $}}
\newcommand{\Wm}  {\mbox{${\rm W}^{\rmsscr {-{\alpha}}} $}}
\newcommand{\W}  {\mbox{${\rm W}^{\rmsscr {\pm}} $}}

\newcommand{\bnumu}      {\mbox{${\bar{\nu}}_{\sscr \mu}$}}
\newcommand{\bnue}       {\mbox{${\bar{\nu}}_{\rm\sscr e}$}}
\newcommand{\bnutau}     {\mbox{${\bar{\nu}}_{\sscr \tau}$}}








